Planar algebra presentations of $\text{URep}_{\mathbb{C}}(\mathbb{C}^+)$ and $\text{URep}_{\mathbb{F}_p}(\mathbb{F}_p^+)$

We give presentations of the planar algebra of unipotent representations of the groups $\mathbb{C}$ and $\mathbb{F}_p$ under addition using jellyfish and light leaf style arguments. These are some of the most natural examples of non-semisimple planar algebras. For the characteristic $p$ family of examples, a new generator appears in arbitrarily large box spaces as $p$ increases. We point toward future directions in getting results on first and second fundamental theorems for rings of vector invariants, as well as generalization of the examples given.

==> compute_p.tex <==
Identify \lcap$\cdots$\lcap$*$\rcap$\cdots$\rcap\hspace{1.5mm}with $j_p:V^{\otimes 2p-1} \rightarrow \mathbbm{1}$, and \dotmap, \lcap\rcap, as in $Alg_0$. We note that $L_{N_p}(n)$ corresponds to the basis $T(Y_n)$ from the previous section. There is an added complication here which doesn't occur in $Alg_0$, which is that we'll want to interpret \lcap$\cdots$\lcap$**$\rcap$\cdots$\rcap\hspace{1.5mm}as two jellyfish stitched together by $p-1$ cups, and similarly whenever we have a sequence of jellyfish stitched together. This amounts to defining the output of $1$ by some number of nested cups, and feeding these factors to the jellyfish legs.


==> rep_pa.tex <==
Consider $Rep_k(G,V)$, the tensor subcategory of $Rep_k(G)$ which is $\otimes$-generated by $V$ and $V^\ast$. We get a planar algebra as follows:
\begin{enumerate}
\item The box space $B_n$ is $Hom(V^{\otimes n} , \mathbbm{1})$.
\item Morphisms of $Rep_k(G,V)$ are labelled boxes, with appropriately oriented incoming and outgoing strands for $Id_V$ and $Id_{V^{\ast}}$. We compose morphisms by gluing outgoing strands of one morphism to incoming strands of another.
\item $\otimes$ product of morphisms corresponds to disjoint union in the planar algebra.
\item To evaluate a picture in the planar algebra, we assume by isotopy all strands are vertical, or a cap/cup (upper/bottom oriented half circle) connecting vertical strands. The cap and cup correspond to the counit and unit morphisms respectively. Then we scan the diagram upwards, applying a morphism to the inputs whenever the diagram has a new feature, i.e. something other than the identity map.
\end{enumerate}

We need to be able to rotate pictures, corresponding to taking the dual morphism, and use the pivotal structure of $Rep_k(G,V)$ to do so. In the case of the unit and counit, the pivotal structure also gives an isomorphism between the left and right dual, so that we always can use evaluation and coevaluation in the case the strand orientation is reversed.
